Lubricated axisymmetric gravity currents of power-law fluids

The motion of glaciers over their bedrock or drops of fluid along a solid surface can become unstable when these substrates are lubricated. Previous studies modeled such systems as coupled gravity currents (GCs) consisting of one fluid that lubricates the flow of another fluid, and having two propagating fronts. When both fluid are Newtonian and discharged at constant flux, global similarity solutions were found. However, when the top fluid is strain-rate softening experiments have shown that each fluid front evolved with a different exponent. Here we explore theoretically and numerically such lubricated GCs in a model that describes the axisymmetric spreading of a power-law fluid on top of a Newtonian fluid, where the discharge of both fluids is power law in time. We find that the model admits similarity solutions only in specific cases, including the purely Newtonian case, for a certain discharge exponent, at asymptotic limits of the fluids viscosity ratio, and at the vicinity of the fluid fronts. Generally, each fluid front has a power-law time evolution with a similar exponent as a non-lubricated GC of the corresponding fluid, and intercepts that depend on both fluid properties. Consequently, we identify two mechanisms by which the inner lubricating fluid front outstrips the outer fluid front. Many aspects of our theory are found consistent with recent laboratory experiments. Discrepancies suggest that hydrofracturing or wall slip may be important near the fronts. This theory may help to understand the dynamics of various systems, including surges and ice streams.

==> packages/bbding/README <==
This directory contains the bbding fontset to be used under LaTeX.  

The original metafont source is written by Karel Horak, which is supposed to have
the copyright for the fonts.  The LaTeX package is written by Peter Møller
Neergaard, which have made some minor changes to the metafont source.
Therefore both the original source and the modified source can be found in
this directory.

The directory contains the following files
	README		This file
	bbding.ins	The installation driver for the LaTeX package
	bbding.dtx	The source for the LaTeX code
	bbding10.mf	The metafont source for the bbding font set with
			some minor corrections to make it work under LaTeX
	bbding10.org	The original metafont source for the bbding font set
	

01/2020

Need to write in \mbox:
$\mbox{\symbol}$

Need to put in the .tex directory the 3 files:

Uding.fd
bbding.sty
bbding10.mf


==> packages/soul/Makefile <==
# $Id: Makefile,v 1.7 2003/06/22 09:23:35 m Rel $

NAME=soul
ARCHNAME=$(NAME).tar.gz
ARCHIVE=$(NAME).dtx Makefile $(NAME).txt $(NAME).ins
MAKEIDXOPT=
DVIPSOPT=#-Pcmz -Pamz
DEP=$(NAME).sty

all: $(NAME).sty $(NAME).ps

print: $(NAME).ps
	psbook $(NAME).ps|psnup -2|psselect -e|lpr
	@ echo -n revert paper stack and hit return
	@ read key
	psbook $(NAME).ps|psnup -2|psselect -o -r|lpr

ps: $(NAME).ps

%.ps: %.dvi
	dvips $(DVIPSOPT) $< -o $@

hyper: $(NAME).dtx $(NAME).sty
	pdflatex "\relax\let\makehyperref\active\input $(NAME).dtx"

$(NAME).pdf: $(NAME).dtx $(NAME).sty
	pdflatex $(NAME).dtx

archive:
	@ tar -czf $(ARCHNAME) $(ARCHIVE)
	@ echo $(ARCHNAME)

clean: 
	rm -f $(NAME).{log,toc,lot,lof,idx,ilg,ind,aux,blg,bbl,dvi,ins,out}

distclean: clean
	rm -f $(NAME).{ps,sty,pdf} $(ARCHNAME)


REFWARN = 'Rerun to get cross-references'
LATEXMAX = 5

%.dvi: %.dtx $(DEP)
	latex $< ; true
	RUNS=$(LATEXMAX); \
	while [ $$RUNS -gt 0 ] ; do \
		if grep $(REFWARN) $*.log > /dev/null; \
		then latex $< ; else break; fi; \
		RUNS=`expr $$RUNS - 1`; \
	done

$(NAME).sty: $(NAME).ins soul.dtx
	tex $(NAME).ins

$(NAME).ins:
	latex $(NAME).dtx


